An Open Source Design Optimization Toolbox Evaluated on a Soft Finger

In this paper, we introduce a novel open source toolbox for design optimization in Soft Robotics. We consider that design optimization is an important trend in Soft Robotics that is changing the way in which designs will be shared and adopted. We evaluate this toolbox on the example of a cable-driven, sensorized soft finger. For devices like these, that feature both actuation and sensing, the need for multi-objective optimization capabilities naturally arises, because at the very least, a trade-off between these two aspects has to be found. Thus, multi-objective optimization capability is one of the central features of the proposed toolbox. We evaluate the optimization of the soft finger and show that extreme points of the optimization trade-off between sensing and actuation are indeed far apart on actually fabricated devices for the established metrics. Furthermore, we provide an in depth analysis of the sim-to-real behavior of the example, taking into account factors such as the mesh density in the simulation, mechanical parameters and fabrication tolerances.

==> Figures/NodesVsVolumeDeformation.tex <==
\definecolor{DeltaV1}{rgb}{0.4,0,0}
\definecolor{DeltaV2}{rgb}{0,0,0.4}
\begin{tikzpicture}
\begin{axis}[
    width=9cm,
    height=5cm,
    title={Number of Nodes vs. Deformation Volume},
    xlabel={\#Nodes},
    ylabel={Vol. Deform. (\si{\micro\liter})},
    xmin=424, xmax=14000,
    ymin=-205, ymax=-50,
    xtick={500, 2500, 4500, 6500, 8500, 11000, 13500},
    ytick={-50,-100,-150,-200},
    ylabel near ticks,
    scaled x ticks = false,
    grid=major,
    legend style = {at={(3,-3)}},
    % legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (484,-68.9)(1030,-96.41)(1885,-158)(2441,-135.3)(3209,-184)(4717,-182.2)(7780,-178.1)(13165,-171.7)    
    };\label{plot1}    
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (484,-58.6)(1030,-80.9)(1885,-153)(2441,-147.4)(3209,-175.27)(4717,-187.17)(7780,-159.4)(13165,-175.2)    
    };\label{plot2}    
\end{axis}
\begin{axis}[
    width=9cm,
    height=5cm,
    axis y line*=right,
    axis x line=none,
    xmin=424, xmax=14000,
    ymin=-0.91, ymax=23.70,
    ytick={0,5,10,15,20},
    ylabel=$\Delta$Vol/$\Delta$\#N (\si{\micro\liter}/\#N)]    

    \addlegendimage{/pgfplots/refstyle=plot1}\addlegendentry{V1}
    \addlegendimage{/pgfplots/refstyle=plot2}\addlegendentry{V2}
    \addplot[
    mark=+,
    dashed,
    color=DeltaV1    
    ]
    coordinates {
    (484,99.6)(1030,5.0)(1885,7.2)(2441,4.1)(3209,6.34)(4717,0.119)(7780,0.133)(13165,0.118)    
    };\label{deltaV1}    
    \addplot[
    mark=+,
    dashed,
    color=DeltaV2    
    ]
    coordinates {
    (484,111.8)(1030,4.1)(1885,8.432)(2441,3.2)(3209,5.2)(4717,0.789)(7780,0.9)(13165,0.3)    
    };\label{deltaV2}    
    \addlegendimage{/pgfplots/refstyle=DeltaV1}\addlegendentry{$\Delta$V1/$\Delta$\#N}
    \addlegendimage{/pgfplots/refstyle=DeltaV2}\addlegendentry{$\Delta$V2/$\Delta$\#N}
\end{axis}
\end{tikzpicture}

==> Figures/SensitivityAnalysis.tex <==
\begin{tikzpicture}
 
\begin{axis} [ybar = 0.05cm,
    bar width = 12pt,
    xmin = -1.5,
    xmax = 4.2,        
    ymin=-0.58, ymax=0.38,
    xticklabels={(a), (a), (b), (c), (d), (e), (f), (g)},
    % xticklabel style = {rotate=45},
    %ytick = data,
    enlarge x limits = {value = .25, upper},
    % legend pos=south west,
    legend style = {at={(0.35,0.23)},anchor=west},
    title={Local Parameter Sensitivity},
    ylabel={Parameter Sensitivity (\%)},
    % grid=major,    
    ymajorgrids=true,
    width=9cm,
    height=5cm,
    % enlarge y limits = {abs = .}
]

\addplot coordinates {(-1,-0.115) (0,0.133) (1,0.076) (2,-0.102) (3,-0.0235) (4,-0.0178) (5,-0.534)};
\addplot coordinates {(-1,0.161) (0,-0.324) (1,0.0372) (2,0.132) (3,-0.028) (4,0.054)(5,0.318)};


 
\legend {Vol. Sens., Ang. Disp.};
 
\end{axis}
 
\end{tikzpicture}
